Feedback Enhanced Motion Planning for Autonomous Vehicles

In this work, we address the motion planning problem for autonomous vehicles through a new lattice planning approach, called Feedback Enhanced Lattice Planner (FELP). Existing lattice planners have two major limitations, namely the high dimensionality of the lattice and the lack of modeling of agent vehicle behaviors. We propose to apply the Intelligent Driver Model (IDM) as a speed feedback policy to address both of these limitations. IDM both enables the responsive behavior of the agents, and uniquely determines the acceleration and speed profile of the ego vehicle on a given path. Therefore, only a spatial lattice is needed, while discretization of higher order dimensions is no longer required. Additionally, we propose a directed-graph map representation to support the implementation and execution of lattice planners. The map can reflect local geometric structure, embed the traffic rules adhering to the road, and is efficient to construct and update. We show that FELP is more efficient compared to other existing lattice planners through runtime complexity analysis, and we propose two variants of FELP to further reduce the complexity to polynomial time. We demonstrate the improvement by comparing FELP with an existing spatiotemporal lattice planner using simulations of a merging scenario and continuous highway traffic. We also study the performance of FELP under different traffic densities.

==> tex/preliminaries.tex <==
\section{Preliminaries}
\label{sec: preliminaries}
In this section, we provide a quick overview of the Intelligent Driver Model (IDM). IDM is an extensively studied topic in the literature of traffic flow modeling. Various IDM~\cite[Ch.11]{treiber2013traffic} are carefully handcrafted so that they model the natural behavior of a driver in lane following. The most basic form of IDM is shown as the following,
\begin{equation}
  \label{eq: intelligent driver model}
  \begin{gathered}
    a =
    \begin{cases}
      \alpha \prl{1 - \left(\frac{v}{v_0}\right)^{4}}, & \text{without leading vehicle},\\
      \alpha \prl{1 - \left(\frac{v}{v_0}\right)^{4} - \left(\frac{s^*}{s}\right)^2}, & \text{with leading vehicle},\\
    \end{cases} \\
    s^* = s_0 + \max\crl{0, vT + \frac{v \Delta v}{2\sqrt{\alpha\beta}}},
  \end{gathered}
\end{equation}
The traffic scenario is delineated by $v$, speed of the target vehicle, $\Delta v$, speed difference between the target vehicle and its leader, and $s$, the following distance. Some hyper-parameters are necessary to model the intrinsics of a target vehicle. $v_0$ is the desired speed. $\alpha$ and $\beta$ are the comfortable acceleration and brake respectively. $s_0$ is the minimum following distance. $T$ is the desired headway. Based on the traffic scenario and the hyper-parameters, $s^*$ is computed as the desired following distance. The final output of the IDM, $a$, is the acceleration to be applied by the target vehicle. In this work, we use the variant of IDM named Adaptive Cruise Control Model (ACC)~\cite[Ch.11.3.8]{treiber2013traffic}. The major advantage of ACC is that less aggressive brake is required in the same scenario compared to Eq.~\eqref{eq: intelligent driver model}.

